Observational and Interventional Causal Learning for Regret-Minimizing Control

We explore how observational and interventional causal discovery methods can be combined. A state-of-the-art observational causal discovery algorithm for time series capable of handling latent confounders and contemporaneous effects, called LPCMCI, is extended to profit from casual constraints found through randomized control trials. Numerical results show that, given perfect interventional constraints, the reconstructed structural causal models (SCMs) of the extended LPCMCI allow 84.6% of the time for the optimal prediction of the target variable. The implementation of interventional and observational causal discovery is modular, allowing causal constraints from other sources. The second part of this thesis investigates the question of regret minimizing control by simultaneously learning a causal model and planning actions through the causal model. The idea is that an agent to optimize a measured variable first learns the system's mechanics through observational causal discovery. The agent then intervenes on the most promising variable with randomized values allowing for the exploitation and generation of new interventional data. The agent then uses the interventional data to enhance the causal model further, allowing improved actions the next time. The extended LPCMCI can be favorable compared to the original LPCMCI algorithm. The numerical results show that detecting and using interventional constraints leads to reconstructed SCMs that allow 60.9% of the time for the optimal prediction of the target variable in contrast to the baseline of 53.6% when using the original LPCMCI algorithm. Furthermore, the induced average regret decreases from 1.2 when using the original LPCMCI algorithm to 1.0 when using the extended LPCMCI algorithm with interventional discovery.

==> src/parts/frontmatter/statement.tex <==
\chapter*{Statement of Authentication}
%\addcontentsline{toc}{chapter}{Statement of Authentication}
\thispagestyle{empty}
% \textbf{English:}
% \\
I hereby declare that I have written the present bachelor's thesis independently, 
without assistance from external parties and without the use of other resources than those indicated. 
The ideas taken directly or indirectly from external sources (including electronic sources) are duly acknowledged in the text.
The material, either in full or in part,
has not been previously submitted for grading at this or any other academic institution.
% \\
% \\
% \textbf{German:}\\
% Hiermit versichere ich, dass ich diese \ifrtype~selbständig mit Unterstützung der Betreuer angefertigt und keine anderen als die angegebenen Quellen und Hilfsmittel verwendet habe.\\
% \ \\
% Die Arbeit oder wesentliche Bestandteile davon sind weder an dieser noch an einer anderen Bildungseinrichtung bereits zur Erlangung eines Abschlusses eingereicht worden.\\
% \ \\
% Ich erkläre weiterhin, bei der Erstellung der Arbeit die einschlägigen Bestimmungen zum Urheberschutz fremder Beiträge entsprechend den Regeln guter wissenschaftlicher Praxis\footnote{Nachzulesen in den DFG-Empfehlungen zur \glqq Sicherung guter wissenschaftlicher Praxis\grqq~bzw. in der Satzung der Universität Stuttgart zur \grqq Sicherung der Integrität wissenschaftlicher Praxis und zum Umgang mit Fehlverhalten in der Wissenschaft\grqq~} eingehalten zu haben. Soweit meine Arbeit fremde Beiträge (z.B. in der Form von Bilder, Zeichnungen, Textpassagen etc.) enthält, habe ich diese Beiträge als solche gekennzeichnet (Zitat, Quellenangabe) und eventuell erforderlich gewordene Zustimmungen der Urheber zur Nutzung dieser Beiträge in meiner Arbeit eingeholt. Mir ist bekannt, dass ich im Fall einer schuldhaften Verletzung dieser Pflichten die daraus entstehenden Konsequenzen zu tragen habe.
\\[2cm]
\parbox{8cm}{
\hrule
\strut \centering\footnotesize Place, date}
\hfill
\parbox{6cm}{
\hrule
\strut \centering\footnotesize \ifrauthor}
\vfill 
\textbf{Examinor: \ifrsupervisor and Dr. Benjamin Unger}
